DragVideo: Interactive Drag-style Video Editing

Video generation models have shown their superior ability to generate photo-realistic video. However, how to accurately control (or edit) the video remains a formidable challenge. The main issues are: 1) how to perform direct and accurate user control in editing; 2) how to execute editings like changing shape, expression, and layout without unsightly distortion and artifacts to the edited content; and 3) how to maintain spatio-temporal consistency of video after editing. To address the above issues, we propose DragVideo, a general drag-style video editing framework. Inspired by DragGAN, DragVideo addresses issues 1) and 2) by proposing the drag-style video latent optimization method which gives desired control by updating noisy video latent according to drag instructions through video-level drag objective function. We amend issue 3) by integrating the video diffusion model with sample-specific LoRA and Mutual Self-Attention in DragVideo to ensure the edited result is spatio-temporally consistent. We also present a series of testing examples for drag-style video editing and conduct extensive experiments across a wide array of challenging editing tasks, such as motion, skeleton editing, etc, underscoring DragVideo can edit video in an intuitive, faithful to the user's intention manner, with nearly unnoticeable distortion and artifacts, while maintaining spatio-temporal consistency. While traditional prompt-based video editing fails to do the former two and directly applying image drag editing fails in the last, DragVideo's versatility and generality are emphasized. Github link: https://github.com/RickySkywalker/DragVideo-Official.

==> tab/fvd_eval.tex <==
\begin{table}
    \centering
    \begin{tabular}{ccccc}
        \toprule
        \small{DragDiff Extension}    & \small{Tune-A-Video}   & \small{DragVideo}  & \small{without LoRA} & \small{without MSA}\\
        \midrule
        400.89            & 2682.37          & \bf 397.43    &  425.42    & 685.15\\
        \bottomrule
    \end{tabular}
    \caption{FVD$\downarrow$ quantitative evaluations}
    \label{tab:fvd_eval}
    \vspace{-22pt}
\end{table}
